MT-Teql: Evaluating and Augmenting Consistency of Text-to-SQL Models with Metamorphic Testing

Text-to-SQL is a task to generate SQL queries from human utterances. However, due to the variation of natural language, two semantically equivalent utterances may appear differently in the lexical level. Likewise, user preferences (e.g., the choice of normal forms) can lead to dramatic changes in table structures when expressing conceptually identical schemas. Envisioning the general difficulty for text-to-SQL models to preserve prediction consistency against linguistic and schema variations, we propose MT-Teql, a Metamorphic Testing-based framework for systematically evaluating and augmenting the consistency of TExt-to-SQL models. Inspired by the principles of software metamorphic testing, MT-Teql delivers a model-agnostic framework which implements a comprehensive set of metamorphic relations (MRs) to conduct semantics-preserving transformations toward utterances and schemas. Model Inconsistency can be exposed when the original and transformed inputs induce different SQL queries. In addition, we leverage the transformed inputs to retrain models for further model robustness boost. Our experiments show that our framework exposes thousands of prediction errors from SOTA models and enriches existing datasets by order of magnitude, eliminating over 40% inconsistency errors without compromising standard accuracy.

==> 5-microbenchmark.tex <==
\section{Microbenchmarks}
\label{sec:micro}
In addition to \S~\ref{sec:test} and \S~\ref{sec:aug}, we further conduct
microbenchmarks to evaluate our work, including 1) naturalness of synthetic
utterances, 2) robustness of augmented models against linguistic variations, and
3) robustness of augmented models against schema variations.

\subsection{Naturalness of Synthetic Utterances}
\label{subsec:naturalness}
As previously mentioned, instead of randomly transforming utterances (e.g.,
replacing certain words with typos) which likely induces ill-formed utterances,
we aim to synthesize \textit{natural} utterances whose incurred inconsistency
likely denotes real-world defects that normal users can encounter. That is, we
advocate the naturalness as an important metric to assess the quality of
synthetic utterances. As there are no well-established metrics to quantify
naturalness, we employ the fluency score~\cite{ge2018fluency} to practically
approximate the naturalness of utterances, which is defined as follows:

\begin{equation}
  f(\boldsymbol{x})=\frac{1}{1+H(\boldsymbol{x})}
\end{equation}

\noindent where $H(\boldsymbol{x})$ is

\begin{equation}
  H(\boldsymbol{x})=-\frac{\sum_{i=1}^{|\boldsymbol{x}|} \log P\left(x_{i} 
  \mid \boldsymbol{x}_{<i}\right)}{|\boldsymbol{x}|}
\end{equation}

\noindent where $P\left(x_{i} \mid \boldsymbol{x}_{<i}\right)$ is the
probability of $x_i$ under given context $\boldsymbol{x}_{<i}$. The overall
fluency scores on synthetic utterances are comparable with original score.
%
We report that the average fluency score on the original utterances is $0.155$
while the average fluency score of synthetic utterances is $0.148$ ($-4.5\%$).

\F~\ref{fig:cdf} further reports the cumulative fluency scores distributions of
original utterances and synthetic utterances. Particularly, in bottom 25\%, the
fluency score distributions of original utterances and synthetic utterances are
very closed, illustrating that our metamorphic relations does not impede the
readability of worse-case utterances in the original dataset too much.

\begin{figure}[!htbp]
\centering
\includegraphics[width=\columnwidth]{fig/cdf.pdf}
\caption{Cumulative fluency scores distributions.}
\label{fig:cdf}
\end{figure}


\input{tab/micro-result.tex}
\subsection{Linguistic Robustness}
\label{subsec:linguistic-robustness}
As we follow the same method to synthesize test cases from \fixme{training set
  and development set}, we also use an external benchmark to evaluate the
generalization ability of proposed augmentation method against complex
linguistic variations. We evaluate the augmented model on ParaphraseBench
(contains 399 hand-crafted utterance on one schema) provided by
DBPal~\cite{weir2020dbpal} to show the robustness of augmented models against
syntactic, morphological, semantic, and lexical variations as well as missing
information in utterances. We report the evaluation results in
\T~\ref{tab:micro-rlt}. 

\subsection{Schema Robustness}
\label{subsec:schema-robustness}
Following ParaphraseBench~\cite{weir2020dbpal}, we also hand craft a benchmark
to evaluate the robustness of models against schema variations. Based on the
original Restaurant schema~\cite{finegan2018improving,popescu2003towards}, we
derive a total of \fixme{30} equivalent schemas.


==> tab/micro-result.tex <==
\begin{table}[!htbp]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l|c|c|c|c|c|c|c|c}
      \hline
    \textbf{Model} & \textbf{NAI}& \textbf{SYN} &\textbf{LEX}&\textbf{MOR}&\textbf{SEM}&\textbf{MIS}&\textbf{MIX}\\
    \thickhline
    SyntaxSQLNet & 17.5 & 14.0&10.5& 5.3& 15.8&15.8&8.8\\\hline
    SyntaxSQLNet+aug & 33.3& 28.1&15.8& 17.5& 26.3& 29.8&24.6\\\hline
    SyntaxSQLNet+RS & 26.3& 15.8&19.3& 15.8& 21.1&15.8&24.6\\\hline
    SyntaxSQLNet+SS &  24.6 &12.2 &8.8& 7.0& 19.3&19.3&17.5\\\hline
    SyntaxSQLNet+AS & 22.8 & 15.8& 10.5& 12.3& 17.5&17.5&17.5\\\thickhline
    IRNet & 70.2& 28.1& 45.6& 42.1& 56.1&47.4&52.6\\\hline
    IRNet+RS & 37.7& 31.6&38.6& 29.8& 43.9&42.1&42.1\\\hline
    IRNet+SS & 63.2& 28.1& 45.6& 29.8& 42.1&46.4&42.1\\\hline
    \fixme{IRNet+AS} & 0& 0&0& 0& 0&0&0\\\hline
    \end{tabular}}
\caption{Inconsistency rate of augmented models on ParaphraseBench.}
\label{tab:micro-rlt}
\end{table}

